The Language of Trauma: Modeling Traumatic Event Descriptions Across Domains with Explainable AI

Psychological trauma can manifest following various distressing events and is captured in diverse online contexts. However, studies traditionally focus on a single aspect of trauma, often neglecting the transferability of findings across different scenarios. We address this gap by training language models with progressing complexity on trauma-related datasets, including genocide-related court data, a Reddit dataset on post-traumatic stress disorder (PTSD), counseling conversations, and Incel forum posts. Our results show that the fine-tuned RoBERTa model excels in predicting traumatic events across domains, slightly outperforming large language models like GPT-4. Additionally, SLALOM-feature scores and conceptual explanations effectively differentiate and cluster trauma-related language, highlighting different trauma aspects and identifying sexual abuse and experiences related to death as a common traumatic event across all datasets. This transferability is crucial as it allows for the development of tools to enhance trauma detection and intervention in diverse populations and settings.

==> latex/figures/all_concepts_counseling.tex <==
-- CONCEPT 0 --
My boyfriend lost his dad\\
 shot and killed my rapist\\
 my mom. My dad\\
 his wife. My uncle\\
 His mom, my grandma\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>
-- CONCEPT 1 --
 My boyfriend and I hit\\
 university was my savior.\\
ogue about how to discuss\\
 ask more questions about what\\
I was raped a couple\\
 Some relaxation and meditation exercises\\
 to decide what to do\\
 have to do to prepare\\
 you will need to encourage\\
 may choose not to discuss\\
 ask questions to focus on\\
 If you want to discuss\\
 how to feel about it\\
 sure what to feel to\\
 may want to consider seeing
-- CONCEPT 2 --
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>
-- CONCEPT 3 --
 perhaps unrealistic expectations of what\\
 to feel may be of\\
 you feel are normal responses\\
 what others may think of\\
 to understand what may be\\
 can feel really good about\\
 sure what to feel to\\
 know what to say to\\
 know what to do about\\
 Try to understand what\\
 how to feel about it\\
 to decide what to do\\
 know what to say if\\
 what you are thinking or\\
 approach is to understand why
-- CONCEPT 4 --
My boyfriend lost his dad\\
 my mom. My dad\\
 shot and killed my rapist\\
 His mom, my grandma\\
My dad cheated on my\\
 I lost my mother recently\\
 his wife. My uncle\\
, my mother and father\\
I was kidnapped at fourteen\\
. My father cheated on\\
My ex-wife married\\
 niece whom my sister abandoned\\
My daughter was overly tired\\
 my mom. Years later\\
 misses mom and dad in
-- CONCEPT 5 --
My boyfriend lost his dad\\
 my mom. My dad\\
 shot and killed my rapist\\
 his wife. My uncle\\
 His mom, my grandma\\
My dad cheated on my\\
 I lost my mother recently\\
, my mother and father\\
. My father cheated on\\
My ex-wife married\\
I was kidnapped at fourteen\\
 Post Traumatic Stress Disorder\\
Post Traumatic Stress Disorder\\
 niece whom my sister abandoned\\
 posttraumatic stress disorder due
-- CONCEPT 6 --
My boyfriend lost his dad\\
 my mom. My dad\\
 abusive father and his wife\\
 his wife. My uncle\\
 His mom, my grandma\\
My dad cheated on my\\
 I lost my mother recently\\
, my mother and father\\
I was kidnapped at fourteen\\
 My sister never defended me\\
, my doctor gave me\\
. He bought me a\\
 all of my family left\\
 broken apart after she got\\
 rehabilitation program and got kicked
-- CONCEPT 7 --
 facing problems with my mom\\
 with my parents have caused\\
 to watch my wife have\\
 had boyfriends by now\\
 able to sign my brother\\
I have twin toddlers.\\
 told my parents and action\\
 verbally and to my son\\
 cheated on while pregnant,\\
. The ex-wife\\
 ex-boyfriend�\\
-girlfriend that he was\\
. The child was placed\\
 live with my parents because\\
 3-years married,
-- CONCEPT 8 --
 never seem to shake the\\
 there is little or no\\
 this one doesn't give\\
 and wait until that "\\
 but yet that seems to\\
 this formula sounds, the\\
 and marijuana may take the\\
, cold? What would\\
's likely that either there\\
 if this is normal.\\
 this normal? Should I\\
 again how not good enough\\
 that it is something odd\\
 a little bit more about\\
, this should raise concern
-- CONCEPT 9 --
I was violently raped by\\
 got pregnant by my boyfriend\\
 my baby mother. She\\
 my children's father left\\
I saw my mother cheating\\
I was raped by multiple\\
My girlfriend was abused as\\
 I got raped by my\\
 I just lost my mom\\
 teenager. My entire family\\
I was raped repeatedly when\\
My grandma and brother both\\
 parents injured my brother,\\
, my husband mentally abused\\
My mother has Alzheimer's


==> latex/figures/all_concepts_ptsd.tex <==
-- CONCEPT 0 --
 in the dream with the\\

In this dream,\\
 awake in the dream,\\
I survived veteran suicide.\\
 Or in a dream rel\\
 toxic relationships with men.\\
,500 military sexual assaults\\
 shot and killed himself in\\
 ago I had a dream\\
 only dated for a few\\
 after having a dream that\\
harmed while in a\\
 was a dream. This\\
 shot herself in the head\\
, on a medical discharge
-- CONCEPT 1 --
 statistics.</s><pad><pad>\\
 I’m rever\\
 advice!</s><pad><pad>\\
 first post, so bear\\
eless</s><pad><pad><pad>\\
 don't understand that haunt\\


While all this\\
 would be appreciated, thanks\\
�t really much point\\
't get me wrong,\\
 could be understood, my\\
, TL;DR martial\\
 here</s><pad><pad><pad>\\
 of my own shadow...\\
't mind me posting this
-- CONCEPT 2 --
 comparing rape victims to animals\\
 Needed in Suicide Prevention\\
 an infestation of evil\\
 movie The Exorcist\\
 treat PTSD in Vietnam Veterans\\
 look up creepy images online\\
A be a zombie.\\
 for PTSD in Veterans \\
 fetal alcohol syndrome children while\\
,500 military sexual assaults\\
land firefighter. PTSD in\\
 physically abused as a toddler\\
 I have been having herpes\\
  It's breast cancer\\
man  as a child
-- CONCEPT 3 --
 gained full custody. When\\
 inpatient stays with psychiatric\\
 to an psychiatric hold for\\
 impregnated. \\
;m, tried on\\
 out of foster care'\\
 monogamous relationships. I\\
 a BDSM dungeon to\\
 telling a parent that their\\
 a child psychiatric unit and\\
 the hospital. It�\\
 weeks in residential treatment,\\
 in acute inpatient for\\
 Outpatient Treatment (A\\
 used as a sex object
-- CONCEPT 4 --
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>\\
<s><s><s><s><s>
-- CONCEPT 5 --
. Our car clipped the\\
 his car multiple times.\\
 my skull. It wasn\\
 raped at least three times\\
 hit another car, causing\\
 22 year old man (\\
 were later found and her\\
 a lot of death,\\
SA and death

\\
 of sexual abuse, two\\
 murder-suicides each\\
 tried to apprehend the two\\
/SuicideWatch and\\
 after service. Fires are\\
 experiences with SSRIs
-- CONCEPT 6 --
 my parents were kids,\\
 my childhood over to my\\
 my mom divorced my violent\\
 I was a child,\\
 had an abusive ex and\\
 my mother died 2 years\\
 memories of my childhood,\\
 abusive and cheating gay ex\\
 first serious boyfriend repeatedly d\\
 realize TW: Childhood sexual\\
 my trauma from childhood,\\
 my now ex of 4\\
 My parents were divorced when\\
 my parents raised me and\\
 throughout my childhood by my
-- CONCEPT 7 --
 some recommendations on books that\\
, and m rated game\\
 from these illnesses rather than\\
 if I ate better,\\
 me advice on what medications\\
 to stick to dehydration as\\
 three restaurants but none of\\
 these ailments have been holding\\
 stem from a specific incidence\\
 drugged me as well\\
 of sleep deprivation, fix\\
 drugged or drunk during\\
 likes anime too) that\\
 because of my symptoms since\\
 virtual reality exposure therapy,
-- CONCEPT 8 --
 extremely frequent flashbacks the first\\
 me bad. The flashbacks\\
 When I was molested\\
 have vivid flashbacks. All\\
aphobia in the last\\
 about flashbacks.
I\\
 phobia related to the\\
 after i was sexually assaulted\\
 young child, was sexually\\
 having nightmares and flashbacks the\\
 repressed memories are a\\
 because I have flashbacks several\\
 always thought the memories were\\
 of scolding via email\\
 like I was abused.
-- CONCEPT 9 --
 dreams about my abuser,\\
 I’m rever\\
 apologized so much, but\\
 in trouble also, so\\
�, because trust me\\
 advice!</s><pad><pad>\\
ing my old else,\\
zac for a totally unrelated\\
eless</s><pad><pad><pad>\\
�t really much point\\
 story short, my abuser\\
 been trying to woke on\\
 first post, so bear\\
 was looking for clarification on\\
 at explaining this, but

==> latex/figures/old_figure_samples_concepts.tex <==

\begin{figure*}[ht]
\newcommand{\boxwidth}[0]{5.5cm}
\newcommand{\fixheightbox}[1]{
  \begin{minipage}[t][8cm][t]{\textwidth}
   \parbox{\boxwidth}{\setlength{\baselineskip}{0.9\baselineskip}
   #1}
  \end{minipage}
}

\newcommand{\highlight}[1]{\colorbox{yellow}{#1}}

\begin{minipage}[t]{0.48\textwidth}
    \centering
    \include{latex/figures/concepts_gtc_small}
    \captionof{figure}{Trauma-related concepts found in the \textbf{GTC Dataset} (Most salient examples, RoBERTa Model)\label{fig:conceptgtc}}
\end{minipage}\hfill
\begin{minipage}[t]{0.48\textwidth}\centering
    \include{latex/figures/concepts_ptsd_small}
    \captionof{figure}{Trauma-related concepts found in the \textbf{PTSD Dataset} (Most salient examples, RoBERTa model)\label{fig:conceptptsd}}
\end{minipage}
\end{figure*}

\begin{figure}[ht]
\newcommand{\boxwidth}[0]{5.5cm}
\newcommand{\fixheightbox}[1]{
  \begin{minipage}[t][8cm][t]{\textwidth}
   \parbox{\boxwidth}{\setlength{\baselineskip}{0.9\baselineskip}
   #1}
  \end{minipage}
}

\newcommand{\highlight}[1]{\colorbox{yellow}{#1}}
     \centering
\include{latex/figures/concepts_counselling_small}
 \caption{Trauma-related concepts found in the \textbf{Counseling Dataset} ((Most salient examples, RoBERTa Model)\label{fig:conceptcounsel}}

% \label{fig:conceptstraumagtc_combined}
\end{figure}
